SLIDE: A machine-learning based method for forced dynamic response estimation of multibody systems

In computational engineering, enhancing the simulation speed and efficiency is a perpetual goal. To fully take advantage of neural network techniques and hardware, we present the SLiding-window Initially-truncated Dynamic-response Estimator (SLIDE), a deep learning-based method designed to estimate output sequences of mechanical or multibody systems with primarily, but not exclusively, forced excitation. A key advantage of SLIDE is its ability to estimate the dynamic response of damped systems without requiring the full system state, making it particularly effective for flexible multibody systems. The method truncates the output window based on the decay of initial effects, such as damping, which is approximated by the complex eigenvalues of the systems linearized equations. In addition, a second neural network is trained to provide an error estimation, further enhancing the methods applicability. The method is applied to a diverse selection of systems, including the Duffing oscillator, a flexible slider-crank system, and an industrial 6R manipulator, mounted on a flexible socket. Our results demonstrate significant speedups from the simulation up to several millions, exceeding real-time performance substantially.

==> Commands.tex <==
\usepackage{xcolor}
\usepackage{graphicx} 
\usepackage{listings}
\usepackage{mathtools}
\usepackage{placeins}
\usepackage{todonotes}

\newcommand{\mytodo}[1]{\textbf{\textit{\textcolor{red}{TO DO: #1}}}}
\renewcommand{\note}[1]{\textbf{\textit{\textcolor{blue}{NOTE: #1}}}}
\newcommand{\comment}[1]{\textbf{\textit{\textcolor{gray}{comment: #1}}}}



% command for frames so that they can easily be cahnged! 
\newcommand{\Gframe}{\ensuremath{\mathrm{0}}}
\newcommand{\Rframe}{\ensuremath{\mathrm{R}}}
\newcommand{\Wframe}{\ensuremath{\mathrm{w}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%common abbreviations:
\newcommand{\ba}{\begin{array}{c}} %==>Mechatronische Systeme
\newcommand{\ea}{\end{array}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}

\newcommand{\bi}{\begin{itemize} \itemsep -2pt}
\newcommand{\ei}{\end{itemize}}

\newcommand{\bn}{\begin{enumerate} \itemsep -2pt}
\newcommand{\en}{\end{enumerate}}


%vector/matrix: (3D)
\newcommand{\vr}[3]{\left[\!\! \begin{array}{c} { #1}\vspace{0.1cm} \\ { #2}\vspace{0.1cm} \\ { #3} \end{array} \!\!\right]}
\newcommand{\mr}[9]{\left[\!\! \begin{array}{ccc} #1 & #2 & #3 \vspace{0.1cm}\\ #4 & #5 & #6 \vspace{0.1cm}\\ #7 & #8 & #9  \end{array} \!\!\right]}
\newcommand{\vsix}[6]{\left[\!\! \begin{array}{c} { #1} \\ { #2} \\ { #3} \\ { #4} \\ { #5} \\ { #6} \end{array} \!\!\right]}
\newcommand{\vsixb}[6]{\begin{array}{c} { #1} \\ { #2} \\ { #3} \\ { #4} \\ { #5} \\ { #6} \end{array} }

\newcommand{\vsixs}[6]{ \begin{array}{c} { #1} \\ { #2} \\ { #3} \\ { #4} \\ { #5} \\ { #6} \end{array} }

%vector/matrix: (2D)
\newcommand{\vp}[2]{\left[\!\! \begin{array}{c} { #1} \vspace{0.1cm}\\ { #2} \end{array} \!\!\right]}
\renewcommand{\mp}[4]{\left[\!\! \begin{array}{cc} #1 & #2 \vspace{0.1cm}\\ #3 & #4 \end{array} \!\!\right]}

%use following commands for unique german/english
\newcommand{\eq}[1]{Eq.~(\ref{#1})}
\newcommand{\eqs}[1]{Eqs.\ (\ref{#1})}
\newcommand{\eqq}[1]{(\ref{#1})}
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\mytab}[1]{Table~\ref{#1}}
\newcommand{\litref}[1]{Ref.~\cite{#1}}

\newcommand{\eqdot}{\, .} %use this for a dot at the end of an equation
\newcommand{\eqcomma}{\, ,} %use this for a comma at the end of an equation

\newcommand{\ra}{\rightarrow}

\newcommand{\Rcal}{\mathbb{R}}
\newcommand{\Ccal}{\mathbb{C}}
\newcommand{\Ncal}{\mathbb{N}}

%Vektoren mit v nachgestellt
\newcommand{\av}{\mathbf{a}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\cv}{\mathbf{c}}
\newcommand{\dv}{\mathbf{d}}
\newcommand{\ev}{\mathbf{e}}
\newcommand{\fv}{\mathbf{f}}
\newcommand{\gv}{\mathbf{g}}

\newcommand{\hv}{\mathbf{h}}
\newcommand{\iv}{\mathbf{i}}
\newcommand{\jv}{\mathbf{j}}

\newcommand{\kv}{\mathbf{k}}
\newcommand{\mv}{\mathbf{m}}
\newcommand{\nv}{\mathbf{n}}
\newcommand{\ov}{\mathbf{o}}
\newcommand{\pv}{\mathbf{p}}
\newcommand{\qv}{\mathbf{q}}
\newcommand{\rv}{\mathbf{r}}
\newcommand{\sv}{\mathbf{s}}
\newcommand{\tv}{\mathbf{t}}
\newcommand{\uv}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\wv}{\mathbf{w}}
\newcommand{\xv}{\mathbf{x}}
\newcommand{\yv}{\mathbf{y}}
\newcommand{\zv}{\mathbf{z}}
\newcommand{\Fv}{\mathbf{F}}
\newcommand{\Mv}{\mathbf{M}}

%Matrizen mit m nachgestellt
\newcommand{\Am}{\mathbf{A}}
\newcommand{\Bm}{\mathbf{B}}
\newcommand{\Cm}{\mathbf{C}}
\newcommand{\Dm}{\mathbf{D}}
\newcommand{\Em}{\mathbf{E}}
\newcommand{\Gm}{\mathbf{G}}
\newcommand{\Hm}{\mathbf{H}}
\renewcommand{\Im}{\mathbf{I}}
\newcommand{\Jm}{\mathbf{J}}
\newcommand{\Km}{\mathbf{K}}
\newcommand{\Lm}{\mathbf{L}}
\newcommand{\Mm}{\mathbf{M}}
\newcommand{\Nm}{\mathbf{N}}
\newcommand{\Qm}{\mathbf{Q}}
\newcommand{\Pm}{\mathbf{P}}
\newcommand{\Rm}{\mathbf{R}}
\newcommand{\Sm}{\mathbf{S}}
\newcommand{\Tm}{\mathbf{T}}
\newcommand{\Um}{\mathbf{U}}
\newcommand{\Vm}{\mathbf{V}}
\newcommand{\Wm}{\mathbf{W}}
\newcommand{\Xm}{\mathbf{X}}

\newcommand{\Rot}{\mathbf{A}}
\newcommand{\dd}{\mathrm{d}}

\newcommand{\co}{\mathrm{c}}
%\newcommand{\si}{\mathrm{s}}

\newcommand{\tp}{^\mathrm{T}} %transpose

\newcommand{\Null}{\mathbf{0}}

%griechische Buchstaben immer mit 't' vorgestellt
%\newcommand{\ttheta}{\mbox{\boldmath $\theta$ \unboldmath}\!\!}
%\newcommand{\tomega}{\mbox{\boldmath $\omega$ \unboldmath}\!\!}
\newcommand{\tomega}{\mbox{$\pmb{\omega}$}\!\!}
\newcommand{\ttheta}{\mbox{$\pmb{\theta}$}\!\!}
\newcommand{\tTheta}{\mbox{$\pmb{\Theta}$}\!}
\newcommand{\tzeta}{\mbox{$\pmb{\zeta}$}\!\!}
\newcommand{\tmu}{\mbox{$\pmb{\mu}$}\!\!}
\newcommand{\txi}{\mbox{$\pmb{\xi}$}\!\!}


\newcommand{\tpsi}{\mbox{\boldmath $\psi$ \unboldmath}\!\!}
\newcommand{\tphi}{\mbox{\boldmath $\phi$ \unboldmath}\!\!}
\newcommand{\talpha}{\mbox{\boldmath $\alpha$ \unboldmath}\!\!}
\newcommand{\tbeta}{\mbox{\boldmath $\beta$ \unboldmath}\!\!}
\newcommand{\tgamma}{\mbox{\boldmath $\gamma$ \unboldmath}\!\!}
%\newcommand{\tlambda}{\mbox{\boldmath $\lambda$ \unboldmath}\!\!}
\newcommand{\tlambda}{\lambda \hspace{-6.4pt} \lambda\hspace{-6.4pt} \lambda}
%\newcommand{\ttau}{\mbox{\boldmath $\tau$ \unboldmath}\!\!}
\newcommand{\ttau}{\ensuremath{\normalsize \tau \hspace{-6.2pt} \tau\hspace{-6.2pt}\tau\hspace{-6.2pt} \tau}}

\newcommand{\tsigma}{\mbox{\boldmath $\sigma$ \unboldmath}\!\!}
\newcommand{\teps}{\mbox{\boldmath $\varepsilon$ \unboldmath}\!\!}
\newcommand{\tnu}{\mbox{\boldmath $\nu$ \unboldmath}\!\!}
%\newcommand{\tmu}{\mbox{\boldmath $\mu$ \unboldmath}\!\!}
\newcommand{\tPhi}{\mbox{\boldmath $\Phi$ \unboldmath}\!\!}
%\newcommand{\tzeta}{\mbox{\boldmath $\zeta$ \unboldmath}\!\!}

\newcommand{\vareps}{\varepsilon}

%left index:
%\newcommand{\LU}[2]{{^{#1}#2}\,}
\newcommand{\LU}[2]{\prescript{#1}{}{#2}\,}
\newcommand{\RL}[2]{\prescript{}{}{#1}_{#2}\,}
\newcommand{\LUR}[3]{\prescript{#1}{}{#2}_{#3}\,}
\newcommand{\LURU}[4]{\prescript{#1}{}{#2}_{#3}^{#4}\,}
\newcommand{\LLdot}[3]{\prescript{}{#1}{\dot{#2}}_{#3}\,}
\newcommand{\sysG}[1]{\LU{\Gframe}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{8} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{8}  % for normal

% Custom colors
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}
\definecolor{commentgreen}{RGB}{78,154,6}
\definecolor{backcolour}{rgb}{0.97,0.97,0.97}


\usepackage{tabularx}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\newcommand{\innerproduct}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\Point}[1]{\ensuremath{\mathrm{P}_\mathrm{#1}}}
%\defincecolor{commentgreen}{0,0.5,0}


%\usepackage{nameref} # referance by name instead of number; unused. 
%\usepackage{siunitx}

% Python style for highlighting
\newcommand\pythonstyle{\lstset{
language=Python,
basicstyle=\ttm,
otherkeywords={self},             % Add keywords here
keywordstyle=\ttb\color{deepblue},
emph={AddNode, AddObject, AddMarker, AddLoad, AddSensor, SystemContainer, 
AddSystem, Assemble, SimulationSettings,
StartRenderer, StopRenderer, GetNodeOutput, function, 
TimeIntegrationSolve,__init__},          % Custom highlighting
emphstyle=\ttb\color{deepred},    % Custom highlighting style
stringstyle=\color{deepgreen},
commentstyle=\color{commentgreen},
%frame=none,                         % horizontal line top and bottom
%frame=tb,                         % horizontal line top and bottom
frame = single,
rulecolor=\color{black}, 		% enforces black frame with 2 lines 
showstringspaces=false,           % 
numbers=left,										 %show line numbers
breaklines=true,									 %automatically breaks lines
numberstyle=\ttm,    						% line number style
backgroundcolor=\color{backcolour}
}}


% Python environment
\lstnewenvironment{python}[1][]
{
\pythonstyle
\lstset{#1}
}
{}

% Python for external files
\newcommand\pythonexternal[2][]{{
\pythonstyle
\lstinputlisting[#1]{#2}}}

% Python for inline
\newcommand\pythoninline[1]{{\pythonstyle\lstinline!#1!}}

\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
						

\newcommand{\tikzpicAnnotate}[4]{
{}{}{}
\begin{tikzpicture}
	\node[above right, inner sep=0] (image) at (0,0) {
    \includegraphics[width=\columnwidth]{#1}
};
\node [anchor=south west] (note) at (#3,#4) {#2};
\end{tikzpicture}
}	

\newcommand{\minipageFig}[3]{
%note (#1)
\begin{minipage}[c]{#1\columnwidth}
%abc
\tikzpicAnnotate{#2}{#3}{0}{0}
\end{minipage}
}

\usepackage{cancel}

%%%%%%%%%%%%%%%%%%%% includes by martin 
\newcommand{\martin}[1]{\todo[color=green!50, inline, caption={}]{[MARTIN          ] #1}}
\newcommand{\martinTodo}[1]{\todo[color=green!50, caption={}]{[MARTIN          ] #1}}

% new commands as makros to be consistent
\newcommand{\RC}{RoboCup}
\newcommand{\RCAW}{RoboCup@Work}
\newcommand{\leobot}{LeoBot}
\newcommand{\MW}{Mecanum wheel}
\newcommand{\MWs}{Mecanum wheels}
\newcommand{\stanford}{Stanford Robotics Platform}
\newcommand{\kairos}{Kairos}
\newcommand{\configOne}{$\mathrm{c}_1$}
\newcommand{\configTwo}{$\mathrm{c}_2$}
\newcommand{\configThree}{$\mathrm{c}_3$}
\newcommand{\configFour}{$\mathrm{c}_4$}
